Synthetic 1-Categories in Directed Type Theory

The field of directed type theory seeks to design type theories capable of reasoning synthetically about (higher) categories, by generalizing the symmetric identity types of Martin-L\"of Type Theory to asymmetric hom-types. We articulate the directed type theory of the category model, with appropriate modalities for keeping track of variances and a powerful directed-J rule capable of proving results about arbitrary terms of hom-types; we put this rule to use in making several constructions in synthetic 1-category theory. Because this theory is expressed entirely in terms of generalized algebraic theories, we know automatically that this directed type theory admits a syntax model and is the first step towards directed higher observational type theory.

==> content/defn/1-1-trunc-DCwF.tex <==
%% ./content/defn/1-1-trunc-DCwF.tex
%%
%% By Jacob Neumann (jacobneu.github.io)
%% October 2024
%%
A \keyword{$(1,1)$-truncated DCwF} is a DCwF such that
\begin{itemize}
\item $\hom(t,t')$ is a \textit{neutral type} for any terms $t,t'$; and
\item UIP holds for identities of hom-terms:
\[ \mathsf{UIP}^1 \colon (\alpha\colon\Tm(\Gamma,\Id(p,q)^-)) \to (\beta\colon\Tm(\Gamma,\Id(p,q))) \to \Tm(\Gamma,\Id(\alpha,\beta)) \]
\end{itemize}


==> content/defn/DCwF.tex <==
%% ./content/defn/DCwF.tex
%%
%% By Jacob Neumann (jacobneu.github.io)
%% October 2024
%%
A \keyword{directed CwF (DCwF)} is a NPCwF equipped with the following structure:
\begin{itemize}
\item a type former $$ \hom \colon \{\Gamma\colon\Con\}\{A\colon\Ty\;\Gamma\} \to \Tm(\Gamma,A^-) \to \Tm(\Gamma,A) \to \Ty\;\Gamma $$ which is stable under substitution: $$\hom(t,t')[\sigma]\equiv\hom(t[\sigma],t'[\sigma]);$$
\item in any $\Gamma\colon\NCon$, a term $\refl_t\colon\hom(t,-t)$ for each term $t\colon\Tm(\Gamma,A^-)$, also stable under substitution by $\sigma\colon\Sub\;\Delta\;\Gamma$ for $\Delta\colon\NCon$; and
\item a term former $\mathsf{J}$ as given in \autoref{tag:dirJ}, also appropriately stable under substitution.
\end{itemize}
For any $\Gamma\colon\Con$ and $A\colon\NTy\;\Gamma$, write $\Id(t,t')$ for $\hom(t,t')$.


==> content/defn/NPCwF.tex <==
%% ./content/defn/NPCwF.tex
%%
%% By Jacob Neumann (jacobneu.github.io)
%% October 2024
%%
A \keyword{sub-PCwF} $\mc D$ of a PCwF $\mc C$ consists of predicates $\mathsf{D}_{\Con}\colon\Con\to\PROP$ and $\mathsf{D}_{\Ty}\colon \{\Gamma\colon\Con\}\to \Ty\;\Gamma\to\PROP$ such that
\begin{itemize}
\item $\mathsf{D}_{\Con}\;\Empty$;
\item if $\mathsf{D}_{\Con}(\Gamma)$, then $\mathsf{D}_{\Con}(\Gamma^-)$;
\item if $\mathsf{D}_{\Ty}(A)$, then $\mathsf{D}_{\Ty}(A^-)$;
\item if $A\colon\Ty\;\Gamma$ is such that $\mathsf{D}_\Ty(A)$, then $\mathsf{D}_\Ty(A[\sigma])$ for any $\sigma\colon\Sub\;\Delta\;\Gamma$; and
\item if $\mathsf{D}_{\Con}(\Gamma)$ and $\mathsf{D}_{\Ty}(A)$, then $\mathsf{D}_{\Con}(\Gamma\cExtend A)$.
\end{itemize}
We indicate a sub-PCwF by $\mc D=(\mathsf{DCon},\mathsf{DTy})$ to indicate that $\mathsf{DCon}$ is the subcategory of $\mathsf{D}_{\Con}$-contexts, and $\mathsf{DTy}$ is the subpresheaf of $\mathsf{D}_{\Ty}$-types.

A \keyword{neutral-polarized category with families (NPCwF)} consists of a PCwF $\mc C$ and a sub-PCwF $\mc N=(\NCon,\NTy)$ such that
\begin{itemize}
\item $\NCon$ is symmetric: every $\Gamma\colon\NCon$ comes equipped with an $e\colon\Sub\;\Gamma\;\Gamma^-$ such that $e^-\colon\Sub\;\Gamma^-\;\Gamma$ is an inverse of $e$; moreover, this isomorphism is natural in the sense that, for $\Delta,\Gamma\colon\NCon$ and $\sigma\colon\Sub\;\Delta\;\Gamma$, we have $\sigma\equiv e^-_{\Gamma}\circ \sigma^- \circ e_{\Delta}$;
\item if either $\Gamma\colon\NCon$ and $A\colon\Ty\;\Gamma$ or $\Gamma\colon\Con$ and $A\colon\NTy\;\Gamma$, there are coercion operations $-\colon\Tm(\Gamma,A) \to \Tm(\Gamma,A^-)$ and $-\colon\Tm(\Gamma,A^-) \to \Tm(\Gamma,A)$ such that $-(-t)\equiv t$ for all $t$;
\item for every $\Gamma\colon\NCon$ and $A\colon\Ty\Gamma^-$, there is an isomorphism $$ (e\cExtend A) \colon \Gamma\cExtend[+] A[e] \cong \Gamma\cExtend[-]A $$ such that
\begin{itemize}
\item $\pp_{-,A} \circ (e\cExtend A) \equiv \pp_{A[e]}$
\item for every $\Delta,\Gamma\colon\NCon$, $\sigma\colon\Sub\;\Delta\;\Gamma$, $A\colon\Ty(\Gamma^-)$ and every  $a\colon\Tm(\Delta,A[e\circ\sigma])$,\footnote{ Note that $e_{\Gamma}\circ \sigma \equiv \sigma^-\circ e_{\Delta}$, so $a\colon\Tm(\Delta,A[\sigma^-\circ e_{\Delta}])$, hence why the right-hand side of the following equation is well-formed. The need for $e_{\Delta}$ and the need to negate $a[e^-]$ is why $\Delta$ must be neutral here.}$$(e\cExtend A)\circ \pair{\sigma,_+ a} \equiv \pair{\sigma,_- -a[e^-]}.$$
\end{itemize}
\end{itemize}



==> content/defn/PCwF.tex <==
%% ./content/defn/PCwF.tex
%%
%% By Jacob Neumann (jacobneu.github.io)
%% October 2024
%%
A \keyword{polarized category with families (PCwF)} consists of a CwF $\mc C=(\Con,\Ty,\Tm,\cExtend,\ldots)$ equipped with the following operations.
\begin{itemize}
\item An endofunctor $(\underlines)^-\colon\Con\fTo\Con$ such that $(\Gamma^-)^-\equiv\Gamma$ and $(\sigma^-)^-\equiv\sigma$ for all $\Gamma$ and $\sigma$
\item A natural transformation $(\underlines)^-\colon\Ty\nTo\Ty$ such that $(A^-)^-\equiv A$ for all $A$.
\end{itemize}



==> content/defn/Pi.tex <==
%% ./content/defn/Pi.tex
%%
%% By Jacob Neumann (jacobneu.github.io)
%% October 2024
%%
A PCwF supports \keyword{polarized $\Pi$-types} if it comes equipped with a type former
\[ \Pi \colon (A\colon\Ty\;\Gamma^-) \to \Ty(\Gamma\cExtend[-]A) \to \Ty\;\Gamma \]
which is stable under substitution, along with a natural isomorphism
\[  \code{lam} \colon \Tm(\Gamma\cExtend[-]A, B) \cong \Tm(\Gamma,\Pi(A,B)) \colon \code{app}. \]


